Weakly Supervised Text-to-SQL Parsing through Question Decomposition

Text-to-SQL parsers are crucial in enabling non-experts to effortlessly query relational data. Training such parsers, by contrast, generally requires expertise in annotating natural language (NL) utterances with corresponding SQL queries. In this work, we propose a weak supervision approach for training text-to-SQL parsers. We take advantage of the recently proposed question meaning representation called QDMR, an intermediate between NL and formal query languages. Given questions, their QDMR structures (annotated by non-experts or automatically predicted), and the answers, we are able to automatically synthesize SQL queries that are used to train text-to-SQL models. We test our approach by experimenting on five benchmark datasets. Our results show that the weakly supervised models perform competitively with those trained on annotated NL-SQL data. Overall, we effectively train text-to-SQL parsers, while using zero SQL annotations.

==> old_03_system.tex <==
\section{Overview}
\label{sec:system}

This section presents our solution for generating NLIDB training data using weak supervision. We begin by describing the high-level pipeline, while in \S\ref{sec:data_generation} we review the different modules of our system.

Our system pipeline is presented in Figure~\ref{fig:architecture}. 
It receives as input a set of weakly supervised training examples $\langle x_i, a_i, s_i, D_i \rangle$. Each example consists of an NL question $x_i$ over a target database $D_i$, its answer $a_i$ and $s_i$, the QDMR decomposition of $x_i$. We assume $x_i, a_i, s_i$ are manually annotated.\footnote{In \S\ref{sec:experiments} we further experiment with predicted QDMRs $\hat{s}_i$ generated by an ML model.}
Given an input example, our goal is to synthesize a SQL query $\hat{Q}_i$ that matches the intention of $x_i$ and, in particular, executes to $a_i$, i.e., $\hat{Q}_i(D_i) = a_i$. 
All examples for which a query $\hat{Q}_i(D)=a$ has been synthesized, are then used as supervised NL-SQL training data $\langle x_i,\hat{Q}_i \rangle$. In our experiments (\S\ref{sec:experiments}) we use the synthesized data to fine-tune a pre-trained language model \cite{Raffel2020ExploringTL}. However, our data generation process is completely independent of the supervised machine learning model of choice.

We note that our system's input is comprised entirely of weakly supervised data that can be procured without the use of expert annotators. As described in \S\ref{sec:background}, question-answer annotations can be provided by non-experts, unfamiliar with SQL \cite{pasupat2015compositional, Zhang2013AutomaticallySS, Wang2017SynthesizingHE, Baik2020DuoquestAD}. As for QDMR instances, they can also be crowdsourced to non-experts \cite{Wolfson2020BreakID} or automatically generated using a trained ML model \cite{Shin2021ConstrainedLM, Hasson2021QuestionDW}. 




